Decoherence time of the ground state spin of $V_{B}$ centers in hexagonal boron nitride

The ground-state spin of optically active defects in hexagonal boron nitride (hBN) offers a promising platform for quantum information applications, such as qubits for quantum computing and nanoscale sensing. A key characteristic of a qubit is its decoherence time, as its duration and controllability are critical for practical applications in quantum technologies. In this work, we investigate the electron spin dephasing time of the negatively charged boron vacancies, $V_{B}$ centers, in the hBN lattice by considering the dipolar hyperfine as well as spin-phonon interactions. We employ an approximate method based on the Holstein-Primakoff transformation to take into account a large number of nuclear spins and Debye model to consider the effect of lattice phonons. We show that, in the presence of the dipolar hyperfine interactions, Hahn-echo coherence time of the $V_{B}$ electron spin is approximately $30\: \mathrm{\mu s}$ at room temperature. Our results provide a step forward in understanding the $V_{B}$ defect decoherence in the hBN, which might be used for quantum information applications.

==> dec.tex <==
@book{stoneham2001theory,
  title={Theory of defects in solids: electronic structure of defects in insulators
    and semiconductors},
  author={Stoneham, Arthur Marshall},
  year={2001},
  publisher={Oxford University Press}
}

@Article{Doherty2013,
  author={Marcus W. Doherty and Neil B. Manson and Paul Delaney and Fedor Jelezko
    and J{\~A}¶rg Wrachtrup and Lloyd C.L. Hollenberg},
  journal={Phys. Rep.},
  title={The nitrogen-vacancy colour centre in diamond},
  year={2013},
  month={jul},
  number={1},
  pages={1--45},
  volume={528},
  doi={10.1016/j.physrep.2013.02.001},
  owner={Mehdi Abdi},
  publisher={Elsevier {BV}}
}

@Article{dolde2014high,
  author={Dolde, Florian and Bergholm, Ville and Wang, Ya and Jakobi, Ingmar and
    Naydenov, Boris and Pezzagna, S{\'e}bastien and Meijer, Jan and Jelezko, Fedor
    and Neumann, Philipp and Schulte-Herbr{\"u}ggen, Thomas and others},
  journal={Nat. Commun.},
  title={High-fidelity spin entanglement using optimal control},
  year={2014},
  number={1},
  pages={3371},
  volume={5},
  doi={https://doi.org/10.1038/ncomms4371},
  publisher={Nature Publishing Group}
}

@article{pla2013high,
  title={High-fidelity readout and control of a nuclear spin qubit in silicon},
  author={Pla, Jarryd J and Tan, Kuan Y and Dehollain, Juan P and Lim, Wee H and
    Morton, John JL and Zwanenburg, Floris A and Jamieson, David N and Dzurak,
    Andrew S and Morello, Andrea},
  journal={Nature},
  volume={496},
  number={7445},
  pages={334--338},
  year={2013},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature12011}
}

@article{jelezko2004observation,
  title={Observation of coherent oscillation of a single nuclear spin and realization
    of a two-qubit conditional quantum gate},
  author={Jelezko, Fedor and Gaebel, T and Popa, I and Domhan, M and Gruber, A
    and Wrachtrup, Jorg},
  journal={Phys. Rev. Lett.},
  volume={93},
  number={13},
  pages={130501},
  year={2004},
  publisher={APS},
  doi={https://doi.org/10.1103/PhysRevLett.93.130501}
}

@article{Cai2013,
  author={Jianming Cai and Alex Retzker and Fedor Jelezko and Martin B. Plenio},
  doi={10.1038/nphys2519},
  journal={Nat. Phys.},
  month={jan},
  number={3},
  owner={Mehdi Abdi},
  pages={168--173},
  publisher={Springer Science and Business Media {LLC}},
  title={A large-scale quantum simulator on a diamond surface at room temperature},
  volume={9},
  year={2013},
  bdsk-url-1={https://doi.org/10.1038/nphys2519}
}

@Article{unden2018coherent,
  author={Unden, Thomas and Tomek, Nikolas and Weggler, Timo and Frank, Florian
    and London, Paz and Zopes, Jonathan and Degen, Christian and Raatz, Nicole
    and Meijer, Jan and Watanabe, Hideyuki and others},
  journal={npj Quantum Inf.},
  title={Coherent control of solid state nuclear spin nano-ensembles},
  year={2018},
  number={1},
  pages={39},
  volume={4},
  doi={https://doi.org/10.1038/s41534-018-0089-8},
  publisher={Nature Publishing Group}
}

@article{London2013,
  author={London, P. and Scheuer, J. and Cai, J.-M. and Schwarz, I. and Retzker,
    A. and Plenio, M. B. and Katagiri, M. and Teraji, T. and Koizumi, S. and Isoya,
    J. and Fischer, R. and McGuinness, L. P. and Naydenov, B. and Jelezko, F.},
  doi={10.1103/PhysRevLett.111.067601},
  issue={6},
  journal={Phys. Rev. Lett.},
  month={Aug},
  numpages={5},
  pages={067601},
  publisher={American Physical Society},
  title={Detecting and Polarizing Nuclear Spins with Double Resonance on a Single
    Electron Spin},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.111.067601},
  volume={111},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevLett.111.067601},
  bdsk-url-2={https://doi.org/10.1103/PhysRevLett.111.067601}
}

@Article{Rej2015,
  author={Rej, Ewa and Gaebel, Torsten and Boele, Thomas and Waddington, David
    EJ and Reilly, David J},
  journal={Nat. Commun.},
  title={Hyperpolarized nanodiamond with long spin-relaxation times},
  year={2015},
  pages={8459},
  volume={6},
  bdsk-url-1={https://doi.org/10.1038/ncomms9459},
  doi={https://doi.org/10.1038/ncomms9459},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/ncomms9459}
}

@Article{Healey2021,
  author={Healey, A.J. and Hall, L.T. and White, G.A.L. and Teraji, T. and Sani,
    M.-A. and Separovic, F. and Tetienne, J.-P. and Hollenberg, L.C.L.},
  journal={Phys. Rev. Appl.},
  title={Polarization Transfer to External Nuclear Spins Using Ensembles of Nitrogen-Vacancy
    Centers},
  year={2021},
  month={May},
  pages={054052},
  volume={15},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevApplied.15.054052},
  bdsk-url-2={https://doi.org/10.1103/PhysRevApplied.15.054052},
  doi={10.1103/PhysRevApplied.15.054052},
  issue={5},
  numpages={16},
  publisher={American Physical Society},
  url={https://link.aps.org/doi/10.1103/PhysRevApplied.15.054052}
}

@Article{Fernandez2018a,
  author={Fern{\'a}ndez-Acebal, P. and Rosolio, O. and Scheuer, J. and M{\"u}ller,
    C. and M{\"u}ller, S. and Schmitt, S. and McGuinness, L.P. and Schwarz, I.
    and Chen, Q. and Retzker, A. and Naydenov, B. and Jelezko, F. and Plenio, M.B.},
  journal={Nano Lett.},
  title={Toward Hyperpolarization of Oil Molecules via Single Nitrogen Vacancy
    Centers in Diamond},
  year={2018},
  number={3},
  pages={1882-1887},
  volume={18},
  bdsk-url-1={https://doi.org/10.1021/acs.nanolett.7b05175},
  date-modified={2022-05-15 08:40:28 +0430},
  doi={10.1021/acs.nanolett.7b05175},
  url={https://doi.org/10.1021/acs.nanolett.7b05175}
}

@Article{alvarez2015local,
  author={{\'A}lvarez, Gonzalo A and Bretschneider, Christian O and Fischer, Ran
    and London, Paz and Kanda, Hisao and Onoda, Shinobu and Isoya, Junichi and
    Gershoni, David and Frydman, Lucio},
  journal={Nat. Commun.},
  title={Local and bulk 13C hyperpolarization in nitrogen-vacancy-centred diamonds
    at variable fields and orientations},
  year={2015},
  number={1},
  pages={8456},
  volume={6},
  doi={https://doi.org/10.1038/ncomms9456},
  publisher={Nature Publishing Group}
}

@Article{king2015room,
  author={King, Jonathan P and Jeong, Keunhong and Vassiliou, Christophoros C and
    Shin, Chang S and Page, Ralph H and Avalos, Claudia E and Wang, Hai-Jing and
    Pines, Alexander},
  journal={Nat. Commun.},
  title={Room-temperature in situ nuclear spin hyperpolarization from optically
    pumped nitrogen vacancy centres in diamond},
  year={2015},
  number={1},
  pages={8965},
  volume={6},
  doi={https://doi.org/10.1038/ncomms9965},
  publisher={Nature Publishing Group}
}

@Article{Scheuer2016,
  author={Jochen Scheuer and Ilai Schwartz and Qiong Chen and David Schulze-Sunninghausen
    and Patrick Carl and Peter Hofer and Alexander Retzker and Hitoshi Sumiya and
    Junichi Isoya and Burkhard Luy and Martin B Plenio and Boris Naydenov and Fedor
    Jelezko},
  journal={New J. Phys.},
  title={Optically induced dynamic nuclear spin polarisation in diamond},
  year={2016},
  month={jan},
  number={1},
  pages={013040},
  volume={18},
  bdsk-url-1={https://doi.org/10.1088/1367-2630/18/1/013040},
  date-modified={2022-05-15 08:42:27 +0430},
  doi={10.1088/1367-2630/18/1/013040},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/1367-2630/18/1/013040}
}

@Article{Ivady2020,
  author={Iv{\'a}dy, Viktor and Barcza, Gergely and Thiering, Gerg{\H{o}} and Li,
    Song and Hamdi, Hanen and Chou, Jyh-Pin and Legeza, {\"O}rs and Gali, Adam},
  journal={npj Comput. Mater.},
  title={Ab initio theory of the negatively charged boron vacancy qubit in hexagonal
    boron nitride},
  year={2020},
  pages={41},
  volume={6},
  bdsk-url-1={https://doi.org/10.1038/s41524-020-0305-x},
  doi={https://doi.org/10.1038/s41524-020-0305-x},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41524-020-0305-x}
}

@Article{Gottscholl2020,
  author={Gottscholl, Andreas and Kianinia, Mehran and Soltamov, Victor and Orlinskii,
    Sergei and Mamin, Georgy and Bradac, Carlo and Kasper, Christian and Krambrock,
    Klaus and Sperlich, Andreas and Toth, Milos and others},
  journal={Nat. Mater.},
  title={Initialization and read-out of intrinsic spin defects in a van der Waals
    crystal at room temperature},
  year={2020},
  number={5},
  pages={540--545},
  volume={19},
  bdsk-url-1={https://doi.org/10.1038/s41563-020-0619-6},
  doi={https://doi.org/10.1038/s41563-020-0619-6},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41563-020-0619-6}
}

@article{Kianinia2020,
  author={Kianinia, Mehran and White, Simon and Fr{\"o}ch, Johannes E and Bradac,
    Carlo and Aharonovich, Igor},
  journal={arXiv preprint arXiv:2004.07968},
  title={Engineering spin defects in hexagonal boron nitride},
  url={https://arxiv.org/abs/2004.07968},
  year={2020},
  bdsk-url-1={https://arxiv.org/abs/2004.07968}
}

@Article{gao2022nuclear,
  author={Xingyu Gao and Sumukh Vaidya and Kejun Li and Peng Ju and Boyang Jiang
    and Zhujing Xu and Andres E. Llacsahuanga Allcca and Kunhong Shen and Takashi
    Taniguchi and Kenji Watanabe and Sunil A. Bhave and Yong P. Chen and Yuan Ping
    and Tongcang Li},
  journal={Nat. Mater.},
  title={Nuclear spin polarization and control in a van der Waals material},
  year={2022},
  pages={1024-1028},
  volume={21},
  doi={https://doi.org/10.1038/s41563-022-01329-8},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41563-022-01329-8}
}

@Article{Gottscholl2021,
  author={Andreas Gottscholl and Matthias Diez and Victor Soltamov and Christian
    Kasper and Andreas Sperlich and Mehran Kianinia and Carlo Bradac and Igor Aharonovich
    and Vladimir Dyakonov},
  journal={Sci. Adv.},
  title={Room temperature coherent control of spin defects in hexagonal boron nitride},
  year={2021},
  number={14},
  pages={3630},
  volume={7},
  abstract={Atomic defects in 2D materials show excellent spin coherence time and
    become promising contenders for quantum applications. Optically active spin
    defects are promising candidates for solid-state quantum information and sensing
    applications. To use these defects in quantum applications coherent manipulation
    of their spin state is required. Here, we realize coherent control of ensembles
    of boron vacancy centers in hexagonal boron nitride (hBN). Specifically, by
    applying pulsed spin resonance protocols, we measure a spin-lattice relaxation
    time of 18 microseconds and a spin coherence time of 2 microseconds at room
    temperature. The spin-lattice relaxation time increases by three orders of
    magnitude at cryogenic temperature. By applying a method to decouple the spin
    state from its inhomogeneous nuclear environment the optically detected magnetic
    resonance linewidth is substantially reduced to several tens of kilohertz.
    Our results are important for the employment of van der Waals materials for
    quantum technologies, specifically in the context of high resolution quantum
    sensing of two-dimensional heterostructures, nanoscale devices, and emerging
    atomically thin magnets.},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/sciadv.abf3630},
  bdsk-url-2={https://doi.org/10.1126/sciadv.abf3630},
  doi={10.1126/sciadv.abf3630},
  url={https://www.science.org/doi/abs/10.1126/sciadv.abf3630}
}

@Article{Tabesh2021,
  author={F T Tabesh and Q Hassanzada and M Hadian and A Hashemi and I Abdolhosseini
    Sarsari and M Abdi},
  journal={Quantum Sci. Technol.},
  title={Strain induced coupling and quantum information processing with hexagonal
    boron nitride quantum emitters},
  year={2021},
  month={oct},
  number={1},
  pages={015002},
  volume={7},
  bdsk-url-1={https://doi.org/10.1088/2058-9565/ac2f4d},
  date-modified={2022-05-15 08:42:33 +0430},
  doi={10.1088/2058-9565/ac2f4d},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/2058-9565/ac2f4d}
}

@Article{Johansson2012,
  author={J.R. Johansson and P.D. Nation and Franco Nori},
  journal={Comput. Phys. Commun.},
  title={QuTiP: An open-source Python framework for the dynamics of open quantum
    systems},
  year={2012},
  issn={0010-4655},
  number={8},
  pages={1760-1772},
  volume={183},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0010465512000835},
  bdsk-url-2={https://doi.org/10.1016/j.cpc.2012.02.021},
  date-modified={2022-05-15 08:41:11 +0430},
  doi={https://doi.org/10.1016/j.cpc.2012.02.021},
  keywords={Open quantum systems, Lindblad master equation, Quantum Monte Carlo,
    Python},
  url={https://www.sciencedirect.com/science/article/pii/S0010465512000835}
}

@article{Chen2015,
  author={Chen, Q. and Schwarz, I. and Jelezko, F. and Retzker, A. and Plenio,
    M. B.},
  doi={10.1103/PhysRevB.92.184420},
  issue={18},
  journal={Phys. Rev. B},
  month={Nov},
  numpages={18},
  pages={184420},
  publisher={American Physical Society},
  title={Optical hyperpolarization of $^{13}\mathrm{C}$ nuclear spins in nanodiamond
    ensembles},
  url={https://link.aps.org/doi/10.1103/PhysRevB.92.184420},
  volume={92},
  year={2015},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.92.184420},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.92.184420}
}

@article{Hartmann,
  author={Hartmann, S. R. and Hahn, E. L.},
  doi={10.1103/PhysRev.128.2042},
  issue={5},
  journal={Phys. Rev.},
  month={Dec},
  numpages={0},
  pages={2042--2053},
  publisher={American Physical Society},
  title={Nuclear Double Resonance in the Rotating Frame},
  url={https://link.aps.org/doi/10.1103/PhysRev.128.2042},
  volume={128},
  year={1962},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRev.128.2042},
  bdsk-url-2={https://doi.org/10.1103/PhysRev.128.2042}
}

@Book{Langhoff2012,
  editor={S. Langhoff},
  publisher={Springer Netherlands},
  title={Quantum Mechanical Electronic Structure Calculations with Chemical Accuracy},
  year={2012},
  isbn={9789401101936},
  date={2012-12-06},
  ean={9789401101936},
  owner={Mehdi Abdi},
  pagetotal={449}
}

@Article{Song2010,
  author={Li Song and Lijie Ci and Hao Lu and Pavel B. Sorokin and Chuanhong Jin
    and Jie Ni and Alexander G. Kvashnin and Dmitry G. Kvashnin and Jun Lou and
    Boris I. Yakobson and Pulickel M. Ajayan},
  journal={Nano Lett.},
  title={Large Scale Growth and Characterization of Atomic Hexagonal Boron Nitride
    Layers},
  year={2010},
  pages={3209--3215},
  volume={10},
  date-added={2022-05-15 08:36:32 +0430},
  date-modified={2022-05-15 08:38:59 +0430},
  doi={10.1021/nl1022139}
}

@article{Uhlenbeck1930,
  author={G. E. Uhlenbeck and L. S. Ornstein},
  date-added={2017-08-25 13:48:52 +0000},
  date-modified={2017-08-25 13:49:40 +0000},
  doi={10.1103/PhysRev.36.823},
  journal={Phys. Rev.},
  pages={823},
  title={On the Theory of the Brownian Motion},
  volume={36},
  year={1930},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.36.823}
}

@article{Weissman1988,
  author={M. B. Weissman},
  date-added={2017-08-22 14:08:08 +0000},
  date-modified={2017-08-22 14:09:43 +0000},
  doi={10.1103/RevModPhys.60.537},
  journal={Rev. Mod. Phys.},
  pages={537--571},
  title={1/f noise and other slow, nonexponential kinetics in condensed matter},
  volume={60},
  year={1988},
  bdsk-url-1={https://doi.org/10.1103/RevModPhys.60.537}
}

@article{Bloch1957,
  author={F. Bloch},
  date-added={2017-08-22 13:47:45 +0000},
  date-modified={2017-08-22 13:48:30 +0000},
  doi={10.1103/PhysRev.105.1206},
  journal={Phys. Rev.},
  pages={1206},
  title={Generalized Theory of Relaxation},
  volume={105},
  year={1957},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.105.1206}
}

@article{Paladino2014,
  author={E. Paladino and Y. M. Galperin and G. Falci and B. L. Altshuler},
  date-added={2017-08-22 09:15:04 +0000},
  date-modified={2017-08-22 09:16:42 +0000},
  doi={10.1103/RevModPhys.86.361},
  journal={Rev. Mod. Phys.},
  pages={361--418},
  title={1/f noise: Implications for solid-state quantum information},
  volume={86},
  year={2014},
  bdsk-url-1={https://doi.org/10.1103/RevModPhys.86.361}
}

@article{Yang2017,
  abstract={Decoherence of electron spins in nanoscale systems is important to
    quantum technologies such as quantum information processing and magnetometry.
    It is also an ideal model problem for studying the crossover between quantum
    and classical phenomena. At low temperatures or in light-element materials
    where the spin-orbit coupling is weak, the phonon scattering in nanostructures
    is less important and the fluctuations of nuclear spins become the dominant
    decoherence mechanism for electron spins. Since the 1950s, semi-classical noise
    theories have been developed for understanding electron spin decoherence. In
    spin-based solid-state quantum technologies, the relevant systems are in the
    nanometer scale and nuclear spin baths are quantum objects which require a
    quantum description. Recently, quantum pictures have been established to understand
    the decoherence and quantum many-body theories have been developed to quantitatively
    describe this phenomenon. Anomalous quantum effects have been predicted and
    some have been experimentally confirmed. A systematically truncated cluster-correlation
    expansion theory has been developed to account for the many-body correlations
    in nanoscale nuclear spin baths that are built up during electron spin decoherence.
    The theory has successfully predicted and explained a number of experimental
    results in a wide range of physical systems. In this review, we will cover
    this recent progress. The limitations of the present quantum many-body theories
    and possible directions for future development will also be discussed.},
  author={Yang, Wen and Ma, Wen-Long and Liu, Ren-Bao},
  date-added={2017-08-18 12:33:07 +0000},
  date-modified={2017-08-18 12:33:36 +0000},
  doi={10.1088/0034-4885/80/1/016001},
  journal={Rep. Prog. Phys.},
  journal-full={Reports on progress in physics. Physical Society (Great Britain)},
  number={1},
  pages={016001},
  pmid={27811398},
  pst={ppublish},
  title={Quantum many-body theory for electron spin decoherence in nanoscale nuclear
    spin baths},
  volume={80},
  year={2017},
  bdsk-url-1={http://dx.doi.org/10.1088/0034-4885/80/1/016001}
}

@article{Dobrovitski2003,
  abstract={We demonstrate that the Chebyshev expansion method is a very efficient
    numerical tool for studying spin-bath decoherence of quantum systems. We consider
    two typical problems arising in studying decoherence of quantum systems consisting
    of a few coupled spins: (i) determining the pointer states of the system and
    (ii) determining the temporal decay of quantum oscillations. As our results
    demonstrate, for determining the pointer states, the Chebyshev-based scheme
    is at least a factor of 8 faster than existing algorithms based on the Suzuki-Trotter
    decomposition. For problems of the second type, the Chebyshev-based approach
    is 3-4 times faster than the Suzuki-Trotter-based schemes. This conclusion
    holds qualitatively for a wide spectrum of systems, with different spin baths
    and different Hamiltonians.},
  author={Dobrovitski, V V and {De Raedt}, H A},
  date-added={2017-08-18 10:20:29 +0000},
  date-modified={2017-08-18 10:21:07 +0000},
  doi={10.1103/PhysRevE.67.056702},
  journal={Phys. Rev. E},
  journal-full={Physical review. E, Statistical, nonlinear, and soft matter physics},
  number={5 Pt 2},
  pages={056702},
  pmid={12786317},
  pst={ppublish},
  title={Efficient scheme for numerical simulations of the spin-bath decoherence},
  volume={67},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevE.67.056702}
}

@article{Sousa2003,
  author={R. {de Sousa} and S. {Das Sarma}},
  date-added={2017-08-18 10:01:29 +0000},
  date-modified={2017-08-18 10:02:25 +0000},
  doi={10.1103/PhysRevB.68.115322},
  journal={Phys. Rev. B},
  pages={115322},
  title={Theory of nuclear-induced spectral diffusion: Spin decoherence of phosphorus
    donors in Si and GaAs quantum dots},
  volume={68},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.68.115322}
}

@article{Hanson2007,
  author={R. Hanson and L. P. Kouwenhoven and J. R. Petta and S. Tarucha and L.
    M. K. Vandersypen},
  doi={10.1103/RevModPhys.79.1217},
  journal={Rev. Mod. Phys.},
  month={oct},
  number={4},
  owner={Mehdi Abdi},
  pages={1217},
  publisher={American Physical Society ({APS})},
  title={Spins in few-electron quantum dots},
  volume={79},
  year={2007},
  bdsk-url-1={http://dx.doi.org/10.1103/RevModPhys.79.1217}
}

@article{Witzel2005,
  author={W. M. Witzel and Rogerio de Sousa and S. Das Sarma},
  doi={10.1103/PhysRevB.72.161306},
  journal={Phys. Rev. B},
  month={oct},
  number={16},
  owner={Mehdi Abdi},
  pages={161306},
  publisher={American Physical Society ({APS})},
  title={Quantum theory of spectral-diffusion-induced electron spin decoherence},
  volume={72},
  year={2005},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.72.161306}
}

@article{Lee1985,
  author={Patrick A. Lee and T. V. Ramakrishnan},
  doi={10.1103/RevModPhys.57.287},
  journal={Rev. Mod. Phys.},
  month={apr},
  number={2},
  owner={Mehdi Abdi},
  pages={287--337},
  publisher={American Physical Society ({APS})},
  title={Disordered electronic systems},
  volume={57},
  year={1985},
  bdsk-url-1={http://dx.doi.org/10.1103/RevModPhys.57.287}
}

@article{Degenfeld2014,
  author={Peter Degenfeld-Schonburg and Michael J. Hartmann},
  doi={10.1103/PhysRevB.89.245108},
  journal={Phys. Rev. B},
  month={jun},
  number={24},
  owner={Mehdi Abdi},
  pages={245108},
  publisher={American Physical Society ({APS})},
  title={Self-consistent projection operator theory for quantum many-body systems},
  volume={89},
  year={2014},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.89.245108}
}

@article{Puebla2016,
  author={Ricardo Puebla and Jorge Casanova and Martin B Plenio},
  doi={10.1088/1367-2630/18/11/113039},
  journal={New J. Phys.},
  month={nov},
  number={11},
  owner={Mehdi Abdi},
  pages={113039},
  publisher={{IOP} Publishing},
  title={A robust scheme for the implementation of the quantum Rabi model in trapped
    ions},
  volume={18},
  year={2016},
  bdsk-url-1={http://dx.doi.org/10.1088/1367-2630/18/11/113039}
}

@article{Cai2012,
  author={J-M Cai and B Naydenov and R Pfeiffer and L P McGuinness and K D Jahnke
    and F Jelezko and M B Plenio and A Retzker},
  doi={10.1088/1367-2630/14/11/113023},
  journal={New J. Phys.},
  month={nov},
  number={11},
  owner={Mehdi Abdi},
  pages={113023},
  publisher={{IOP} Publishing},
  title={Robust dynamical decoupling with concatenated continuous driving},
  volume={14},
  year={2012},
  bdsk-url-1={http://dx.doi.org/10.1088/1367-2630/14/11/113023}
}

@article{Khaetskii2003,
  author={Alexander Khaetskii and Daniel Loss and Leonid Glazman},
  doi={10.1103/PhysRevB.67.195329},
  journal={Phys. Rev. B},
  month={may},
  number={19},
  owner={Mehdi Abdi},
  pages={195329},
  publisher={American Physical Society ({APS})},
  title={Electron spin evolution induced by interaction with nuclei in a quantum
    dot},
  volume={67},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.67.195329}
}

@book{Breuer2007,
  author={Heinz-Peter Breuer and Francesco Petruccione},
  date={2007-02-11},
  ean={9780199213900},
  isbn={978-0199213900},
  owner={Mehdi Abdi},
  publisher={Oxford University Press},
  title={The Theory of Open Quantum Systems},
  url={http://www.ebook.de/de/product/6212122/heinz_peter_breuer_francesco_petruccione_the_theory_of_open_quantum_systems.html},
  year={2007},
  bdsk-url-1={http://www.ebook.de/de/product/6212122/heinz_peter_breuer_francesco_petruccione_the_theory_of_open_quantum_systems.html}
}

@Article{Fernandez2018b,
  author={Fern{\'a}ndez-Acebal, P and Plenio, Martin B},
  journal={Sci. Rep.},
  title={Sensing phases of water via nitrogen-vacancy centres in diamond},
  year={2018},
  number={1},
  pages={13453},
  volume={8},
  bdsk-url-1={https://doi.org/10.1038/s41598-018-31745-3},
  date-modified={2022-05-15 08:40:18 +0430},
  doi={10.1038/s41598-018-31745-3}
}

@Article{Holstein1940,
  author={Holstein, T and Primakoff, Hl},
  journal={Phys. Rev.},
  title={Field dependence of the intrinsic domain magnetization of a ferromagnet},
  year={1940},
  number={12},
  pages={1098},
  volume={58},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.58.1098},
  date-modified={2022-05-15 08:41:01 +0430},
  doi={10.1103/PhysRev.58.1098},
  publisher={APS}
}

@Article{Fanchini2014,
  author={Fanchini, Felipe F and Karpat, Goktug and {\c{C}}akmak, Baris and Castelano,
    LK and Aguilar, GH and Far{\'\i}as, O Jim{\'e}nez and Walborn, SP and Ribeiro,
    PH Souto and De Oliveira, MC},
  journal={Phys. Rev. Lett.},
  title={Non-Markovianity through accessible information},
  year={2014},
  number={21},
  pages={210402},
  volume={112},
  date-modified={2022-05-15 08:39:29 +0430},
  publisher={APS}
}

@article{Loretz2017,
  author={Loretz, M. and Takahashi, H. and Segawa, T. F. and Boss, J. M. and Degen,
    C. L.},
  doi={10.1103/PhysRevB.95.064413},
  issue={6},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={6},
  pages={064413},
  publisher={American Physical Society},
  title={Optical hyperpolarization of nitrogen donor spins in bulk diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.95.064413},
  volume={95},
  year={2017},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.95.064413},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.95.064413}
}

@article{Bucher2020,
  author={Bucher, Dominik B. and Glenn, David R. and Park, Hongkun and Lukin, Mikhail
    D. and Walsworth, Ronald L.},
  doi={10.1103/PhysRevX.10.021053},
  issue={2},
  journal={Phys. Rev. X},
  month={Jun},
  numpages={9},
  pages={021053},
  publisher={American Physical Society},
  title={Hyperpolarization-Enhanced NMR Spectroscopy with Femtomole Sensitivity
    Using Quantum Defects in Diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevX.10.021053},
  volume={10},
  year={2020},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevX.10.021053},
  bdsk-url-2={https://doi.org/10.1103/PhysRevX.10.021053}
}

@article{Tetienne2021a,
  author={Tetienne, J.-P. and Hall, L. T. and Healey, A. J. and White, G. A. L.
    and Sani, M.-A. and Separovic, F. and Hollenberg, L. C. L.},
  date-modified={2022-05-15 08:42:50 +0430},
  doi={10.1103/PhysRevB.103.014434},
  issue={1},
  journal={Phys. Rev. B},
  month={Jan},
  numpages={17},
  pages={014434},
  publisher={American Physical Society},
  title={Prospects for nuclear spin hyperpolarization of molecular samples using
    nitrogen-vacancy centers in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.103.014434},
  volume={103},
  year={2021},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.103.014434},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.103.014434}
}

@article{Green2017,
  author={Green, B. L. and Breeze, B. G. and Rees, G. J. and Hanna, J. V. and Chou,
    J.-P. and Iv\'ady, V. and Gali, A. and Newton, M. E.},
  doi={10.1103/PhysRevB.96.054101},
  issue={5},
  journal={Phys. Rev. B},
  month={Aug},
  numpages={8},
  pages={054101},
  publisher={American Physical Society},
  title={All-optical hyperpolarization of electron and nuclear spins in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.96.054101},
  volume={96},
  year={2017},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.96.054101},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.96.054101}
}

@article{Griffin2010,
  author={Griffin, R. G. and Prisner, T. F.},
  doi={10.1039/C0CP90019B},
  issue={22},
  journal={Phys. Chem. Chem. Phys.},
  pages={5737-5740},
  publisher={The Royal Society of Chemistry},
  title={High field dynamic nuclear polarization-the renaissance},
  url={http://dx.doi.org/10.1039/C0CP90019B},
  volume={12},
  year={2010},
  bdsk-url-1={http://dx.doi.org/10.1039/C0CP90019B}
}

@Article{Thankamony2017,
  author={Aany Sofia {Lilly Thankamony} and Johannes J. Wittmann and Monu Kaushik
    and Bjorn Corzilius},
  journal={Prog. Nuc. Mag. Res. Sp.},
  title={Dynamic nuclear polarization for sensitivity enhancement in modern solid-state
    NMR},
  year={2017},
  issn={0079-6565},
  pages={120-195},
  volume={102-103},
  abstract={The field of dynamic nuclear polarization has undergone tremendous
    developments and diversification since its inception more than 6 decades ago.
    In this review we provide an in-depth overview of the relevant topics involved
    in DNP-enhanced MAS NMR spectroscopy. This includes the theoretical description
    of DNP mechanisms as well as of the polarization transfer pathways that can
    lead to a uniform or selective spreading of polarization between nuclear spins.
    Furthermore, we cover historical and state-of-the art aspects of dedicated
    instrumentation, polarizing agents, and optimization techniques for efficient
    MAS DNP. Finally, we present an extensive overview on applications in the fields
    of structural biology and materials science, which underlines that MAS DNP
    has moved far beyond the proof-of-concept stage and has become an important
    tool for research in these fields.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0079656517300201},
  bdsk-url-2={https://doi.org/10.1016/j.pnmrs.2017.06.002},
  doi={https://doi.org/10.1016/j.pnmrs.2017.06.002},
  url={https://www.sciencedirect.com/science/article/pii/S0079656517300201}
}

@Article{Gallagher2008,
  author={Gallagher, Ferdia A and Kettunen, Mikko I and Day, Sam E and Hu, De-En
    and Ardenkjaer-Larsen, Jan Henrik and Zandt, Ren{\'e} and Jensen, Pernille
    R and Karlsson, Magnus and Golman, Klaes and Lerche, Mathilde H and others},
  journal={Nature},
  title={Magnetic resonance imaging of pH in vivo using hyperpolarized ${}^{13}$C-labelled
    bicarbonate},
  year={2008},
  number={7197},
  pages={940--943},
  volume={453},
  bdsk-url-1={{\%}22https://doi.org/10.1038/nature07017{\%}22},
  doi={"https://doi.org/10.1038/nature07017"},
  publisher={Nature Publishing Group},
  url={"https://doi.org/10.1038/nature07017"}
}

@Article{Bowen2008,
  author={Bowen, Sean and Hilty, Christian},
  journal={Angew. Chem. Int. Ed.},
  title={Time-Resolved Dynamic Nuclear Polarization Enhanced NMR Spectroscopy},
  year={2008},
  number={28},
  pages={5235-5237},
  volume={47},
  abstract={The sensitive touch: Sensitivity constraints in NMR spectroscopy typically
    call for long measurement times. Hyperpolarization can enhance the time resolution
    of NMR spectroscopy by removing the need for signal averaging. Reactions such
    as enzyme catalysis can be followed in real time by hyperpolarized NMR spectroscopy
    through reduction in the intensity of the substrate resonance as well as the
    appearance of product resonances (see picture).},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.200801492},
  bdsk-url-2={https://doi.org/10.1002/anie.200801492},
  doi={https://doi.org/10.1002/anie.200801492},
  keywords={enzyme catalysis, hyperpolarization, kinetics, NMR spectroscopy},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.200801492}
}

@Article{Cunningham2016,
  author={Charles H. Cunningham and Justin Y.C. Lau and Albert P. Chen and Benjamin
    J. Geraghty and William J. Perks and Idan Roifman and Graham A. Wright and
    Kim A. Connelly},
  journal={Circ. Res.},
  title={Hyperpolarized ${}^{13}$C Metabolic MRI of the Human Heart},
  year={2016},
  number={11},
  pages={1177-1182},
  volume={119},
  bdsk-url-1={https://www.ahajournals.org/doi/abs/10.1161/CIRCRESAHA.116.309769},
  url={https://www.ahajournals.org/doi/abs/10.1161/CIRCRESAHA.116.309769}
}

@Article{Foletti2009,
  author={Foletti, Sandra and Bluhm, Hendrik and Mahalu, Diana and Umansky, Vladimir
    and Yacoby, Amir},
  journal={Nat. Phys.},
  title={Universal quantum control of two-electron spin quantum bits using dynamic
    nuclear polarization},
  year={2009},
  number={12},
  pages={903--908},
  volume={5},
  bdsk-url-1={{\%}22https://doi.org/10.1038/nphys1424{\%}22},
  doi={"https://doi.org/10.1038/nphys1424"},
  publisher={Nature Publishing Group},
  url={"https://doi.org/10.1038/nphys1424"}
}

@Article{Natterer1997,
  author={Johannes Natterer and Joachim Bargon},
  journal={Prog. Nuc. Mag. Res. Sp.},
  title={Parahydrogen induced polarization},
  year={1997},
  issn={0079-6565},
  number={4},
  pages={293-315},
  volume={31},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0079656597000071},
  bdsk-url-2={https://doi.org/10.1016/S0079-6565(97)00007-1},
  doi={https://doi.org/10.1016/S0079-6565(97)00007-1},
  keywords={PASADENA, PHIP, ALTADENA, Para- and orthohydrogen, Homogeneous hydrogenation,
    Hydrides, Coherence transfer, Hydrogenation mechanisms, Signal enhancement,
    NMR pulse sequences},
  url={https://www.sciencedirect.com/science/article/pii/S0079656597000071}
}

@Article{Hovener2018,
  author={H{\"o}vener, Jan-Bernd and Pravdivtsev, Andrey N. and Kidd, Bryce and
    Bowers, C. Russell and Gl{\"o}ggler, Stefan and Kovtunov, Kirill V. and Plaumann,
    Markus and Katz-Brull, Rachel and Buckenmaier, Kai and Jerschow, Alexej and
    Reineri, Francesca and Theis, Thomas and Shchepin, Roman V. and Wagner, Shawn
    and Bhattacharya, Pratip and Zacharias, Niki M. and Chekmenev, Eduard Y.},
  journal={Angew. Chem. Int. Ed.},
  title={Parahydrogen-Based Hyperpolarization for Biomedicine},
  year={2018},
  number={35},
  pages={11140-11162},
  volume={57},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.201711842},
  bdsk-url-2={https://doi.org/10.1002/anie.201711842},
  doi={https://doi.org/10.1002/anie.201711842},
  keywords={hyperpolarization, magnetic resonance imaging, NMR spectroscopy, parahydrogen},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.201711842}
}

@article{Walker1998,
  author={Walker, Thad G. and Happer, William},
  doi={10.1103/RevModPhys.69.629},
  issue={2},
  journal={Rev. Mod. Phys.},
  month={Apr},
  numpages={0},
  pages={629--642},
  publisher={American Physical Society},
  title={Spin-exchange optical pumping of noble-gas nuclei},
  url={https://link.aps.org/doi/10.1103/RevModPhys.69.629},
  volume={69},
  year={1997},
  bdsk-url-1={https://link.aps.org/doi/10.1103/RevModPhys.69.629},
  bdsk-url-2={https://doi.org/10.1103/RevModPhys.69.629}
}

@Article{Navon1996,
  author={G. Navon and Y.-Q. and T. R{\~o}{\~o}m and S. Appelt and R. E. Taylor
    and A. Pines},
  journal={Science},
  title={Enhancement of Solution NMR and MRI with Laser-Polarized Xenon},
  year={1996},
  number={5257},
  pages={1848-1851},
  volume={271},
  abstract={Optical pumping with laser light can be used to polarize the nuclear
    spins of gaseous xenon-129. When hyperpolarized xenon-129 is dissolved in liquids,
    a time-dependent departure of the proton spin polarization from its thermal
    equilibrium is observed. The variation of the magnetization is an unexpected
    manifestation of the nuclear Overhauser effect, a consequence of cross-relaxation
    between the spins of solution protons and dissolved xenon-129. Time-resolved
    magnetic resonance images of both nuclei in solution show that the proton magnetization
    is selectively perturbed in regions containing spin-polarized xenon-129. This
    effect could find use in nuclear magnetic resonance spectroscopy of surfaces
    and proteins and in magnetic resonance imaging.},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/science.271.5257.1848},
  bdsk-url-2={https://doi.org/10.1126/science.271.5257.1848},
  doi={10.1126/science.271.5257.1848},
  url={https://www.science.org/doi/abs/10.1126/science.271.5257.1848}
}

@article{Villazon2021,
  author={Villazon, Tamiro and Claeys, Pieter W. and Polkovnikov, Anatoli and Chandran,
    Anushya},
  doi={10.1103/PhysRevB.103.075118},
  issue={7},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={21},
  pages={075118},
  publisher={American Physical Society},
  title={Shortcuts to dynamic polarization},
  url={https://link.aps.org/doi/10.1103/PhysRevB.103.075118},
  volume={103},
  year={2021},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.103.075118},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.103.075118}
}

@Article{Abragam1978,
  author={A Abragam and M Goldman},
  journal={Rep. Progr. Phys.},
  title={Principles of dynamic nuclear polarisation},
  year={1978},
  month={mar},
  number={3},
  pages={395--467},
  volume={41},
  abstract={After a general introduction, two sections are devoted to a survey
    of the theories of spin temperature and of nuclear relaxation in solids. This
    is followed by a short section on the so-called well-resolved solid effect,
    and a much more detailed one on DNP by thermal mixing in the non-linear low
    spin-temperature domain. One then analyses the various methods of measurement
    of the nuclear polarisation, as well as an indirect method of detecting the
    electronic resonance based on the existence of large nuclear polarisations.
    The final section describes briefly several applications of dynamic nuclear
    polarisation.},
  bdsk-url-1={https://doi.org/10.1088/0034-4885/41/3/002},
  doi={10.1088/0034-4885/41/3/002},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/0034-4885/41/3/002}
}

@article{Gullans2013,
  author={Gullans, M. and Krich, J. J. and Taylor, J. M. and Halperin, B. I. and
    Lukin, M. D.},
  doi={10.1103/PhysRevB.88.035309},
  issue={3},
  journal={Phys. Rev. B},
  month={Jul},
  numpages={14},
  pages={035309},
  publisher={American Physical Society},
  title={Preparation of nonequilibrium nuclear spin states in double quantum dots},
  url={https://link.aps.org/doi/10.1103/PhysRevB.88.035309},
  volume={88},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.88.035309},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.88.035309}
}

@article{Lai2006,
  author={Lai, C. W. and Maletinsky, P. and Badolato, A. and Imamoglu, A.},
  doi={10.1103/PhysRevLett.96.167403},
  issue={16},
  journal={Phys. Rev. Lett.},
  month={Apr},
  numpages={4},
  pages={167403},
  publisher={American Physical Society},
  title={Knight-Field-Enabled Nuclear Spin Polarization in Single Quantum Dots},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.96.167403},
  volume={96},
  year={2006},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevLett.96.167403},
  bdsk-url-2={https://doi.org/10.1103/PhysRevLett.96.167403}
}

@article{Urbaszek2013,
  author={Urbaszek, Bernhard and Marie, Xavier and Amand, Thierry and Krebs, Olivier
    and Voisin, Paul and Maletinsky, Patrick and H\"ogele, Alexander and Imamoglu,
    Atac},
  doi={10.1103/RevModPhys.85.79},
  issue={1},
  journal={Rev. Mod. Phys.},
  month={Jan},
  numpages={0},
  pages={79--133},
  publisher={American Physical Society},
  title={Nuclear spin physics in quantum dots: An optical investigation},
  url={https://link.aps.org/doi/10.1103/RevModPhys.85.79},
  volume={85},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/RevModPhys.85.79},
  bdsk-url-2={https://doi.org/10.1103/RevModPhys.85.79}
}

@Article{Lee2016,
  author={Daniel Lee and Eric Bouleau and Pierre Saint-Bonnet and Sabine Hediger
    and Ga{\"e}l {De Pa{\"e}pe}},
  journal={J. Magn. Reson.},
  title={Ultra-low temperature MAS-DNP},
  year={2016},
  issn={1090-7807},
  note={Hyperpolarized NMR Comes of Age},
  pages={116-124},
  volume={264},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S1090780715003092},
  bdsk-url-2={https://doi.org/10.1016/j.jmr.2015.12.010},
  doi={https://doi.org/10.1016/j.jmr.2015.12.010},
  keywords={Dynamic nuclear polarization, Magic angle spinning, Solid-state NMR,
    Cryogenic helium, Helium sample spinning},
  url={https://www.sciencedirect.com/science/article/pii/S1090780715003092}
}

@Article{Kaplan2015,
  author={Kaplan, Mohammed and Cukkemane, Abhishek and Van Zundert, Gydo CP and
    Narasimhan, Siddarth and Dani{\"e}ls, Mark and Mance, Deni and Waksman, Gabriel
    and Bonvin, Alexandre MJJ and Fronzes, R{\'e}mi and Folkers, Gert E and others},
  journal={Nat. Methods},
  title={Probing a cell-embedded megadalton protein complex by DNP-supported solid-state
    NMR},
  year={2015},
  number={7},
  pages={649--652},
  volume={12},
  bdsk-url-1={https://doi.org/10.1038/nmeth.3406},
  doi={https://doi.org/10.1038/nmeth.3406},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nmeth.3406}
}

@article{King2010,
  author={King, Jonathan P. and Coles, Patrick J. and Reimer, Jeffrey A.},
  doi={10.1103/PhysRevB.81.073201},
  issue={7},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={4},
  pages={073201},
  publisher={American Physical Society},
  title={Optical polarization of $^{13}\text{C}$ nuclei in diamond through nitrogen
    vacancy centers},
  url={https://link.aps.org/doi/10.1103/PhysRevB.81.073201},
  volume={81},
  year={2010},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.81.073201},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.81.073201}
}

@article{Pagliero2018,
  author={Pagliero, Daniela and Rao, K. R. Koteswara and Zangara, Pablo R. and
    Dhomkar, Siddharth and Wong, Henry H. and Abril, Andrea and Aslam, Nabeel and
    Parker, Anna and King, Jonathan and Avalos, Claudia E. and Ajoy, Ashok and
    Wrachtrup, Joerg and Pines, Alexander and Meriles, Carlos A.},
  doi={10.1103/PhysRevB.97.024422},
  issue={2},
  journal={Phys. Rev. B},
  month={Jan},
  numpages={12},
  pages={024422},
  publisher={American Physical Society},
  title={Multispin-assisted optical pumping of bulk $^{13}\mathrm{C}$ nuclear spin
    polarization in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.97.024422},
  volume={97},
  year={2018},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.97.024422},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.97.024422}
}

@Article{Ajoy2018,
  author={Ashok Ajoy and Kristina Liu and Raffi Nazaryan and Xudong Lv and Pablo
    R. Zangara and Benjamin Safvati and Guoqing Wang and Daniel Arnold and Grace
    Li and Arthur Lin and Priyanka Raghavan and Emanuel Druga and Siddharth Dhomkar
    and Daniela Pagliero and Jeffrey A. Reimer and Dieter Suter and Carlos A. Meriles
    and Alexander Pines},
  journal={Sci. Adv.},
  title={Orientation-independent room temperature optical $^{13}\mathrm{C}$ hyperpolarization
    in powdered diamond},
  year={2018},
  number={5},
  pages={5492},
  volume={4},
  abstract={@Commentjabref-meta: databaseType:bibtex;},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/sciadv.aar5492},
  bdsk-url-2={https://doi.org/10.1126/sciadv.aar5492},
  doi={10.1126/sciadv.aar5492},
  url={https://www.science.org/doi/abs/10.1126/sciadv.aar5492}
}

@article{Abdi2018,
  author={Abdi, Mehdi and Chou, Jyh-Pin and Gali, Adam and Plenio, Martin B.},
  doi={10.1021/acsphotonics.7b01442},
  journal={ACS Photonics},
  number={5},
  pages={1967-1976},
  title={Color Centers in Hexagonal Boron Nitride Monolayers: A Group Theory and
    Ab Initio Analysis},
  url={https://doi.org/10.1021/acsphotonics.7b01442},
  volume={5},
  year={2018},
  bdsk-url-1={https://doi.org/10.1021/acsphotonics.7b01442}
}

@article{Abdi2017,
  author={Mehdi Abdi and Myung-Joong Hwang and Mortaza Aghtar and Martin B. Plenio},
  doi={10.1103/physrevlett.119.233602},
  journal={Phys. Rev. Lett.},
  month={dec},
  number={23},
  owner={Mehdi Abdi},
  pages={233602},
  publisher={American Physical Society ({APS})},
  title={Spin-Mechanical Scheme with Color Centers in Hexagonal Boron Nitride Membranes},
  volume={119},
  year={2017},
  bdsk-url-1={https://doi.org/10.1103/physrevlett.119.233602}
}

@article{Abdi2019,
  author={Mehdi Abdi and Martin B. Plenio},
  date-added={2021-01-16 09:39:24 +0330},
  date-modified={2021-01-16 09:39:24 +0330},
  doi={10.1103/physrevlett.122.023602},
  journal={Phys. Rev. Lett.},
  month={jan},
  number={2},
  pages={023602},
  publisher={American Physical Society ({APS})},
  title={Quantum Effects in a Mechanically Modulated Single-Photon Emitter},
  volume={122},
  year={2019},
  bdsk-url-1={https://doi.org/10.1103/physrevlett.122.023602}
}

@Article{Henshaw2019,
  author={Henshaw, Jacob and Pagliero, Daniela and Zangara, Pablo R. and Franzoni,
    Mar{\'\i}a B. and Ajoy, Ashok and Acosta, Rodolfo H. and Reimer, Jeffrey A.
    and Pines, Alexander and Meriles, Carlos A.},
  journal={Proc. Natl. Acad. Sci.},
  title={Carbon-13 dynamic nuclear polarization in diamond via a microwave-free
    integrated cross effect},
  year={2019},
  issn={0027-8424},
  number={37},
  pages={18334--18340},
  volume={116},
  abstract={Optical spin pumping of color centers promises to revolutionize the
    practice of nuclear magnetic resonance via efficient dynamic nuclear polarization
    protocols. Significant progress has been attained with systems such as the
    nitrogen-vacancy (NV) center in diamond, but extreme spectral broadening and
    nuclear spin-lattice relaxation from coexisting paramagnetic defects are hurdles
    still difficult to circumvent. The present technique addresses both issues
    through the implementation of magnetic-field-sweep{\textendash}induced NV cross-relaxation
    with ancilla point defects, here acting as proxies to mediate the transfer
    of polarization to the nuclear spin ensemble. The governing spin dynamics is
    robust to field misalignment and ideally suited for shallow NVs, indirectly
    coupled to outside nuclei through paramagnetic defects at the diamond surface.Color-center{\textendash}hosting
    semiconductors are emerging as promising source materials for low-field dynamic
    nuclear polarization (DNP) at or near room temperature, but hyperfine broadening,
    susceptibility to magnetic field heterogeneity, and nuclear spin relaxation
    induced by other paramagnetic defects set practical constraints difficult to
    circumvent. Here, we explore an alternate route to color-center{\textendash}assisted
    DNP using nitrogen-vacancy (NV) centers in diamond coupled to substitutional
    nitrogen impurities, the so-called P1 centers. Working near the level anticrossing
    condition{\textemdash}where the P1 Zeeman splitting matches one of the NV spin
    transitions{\textemdash}we demonstrate efficient microwave-free 13C DNP through
    the use of consecutive magnetic field sweeps and continuous optical excitation.
    The amplitude and sign of the polarization can be controlled by adjusting the
    low-to-high and high-to-low magnetic field sweep rates in each cycle so that
    one is much faster than the other. By comparing the 13C DNP response for different
    crystal orientations, we show that the process is robust to magnetic field/NV
    misalignment, a feature that makes the present technique suitable to diamond
    powders and settings where the field is heterogeneous. Applications to shallow
    NVs could capitalize on the greater physical proximity between surface paramagnetic
    defects and outer nuclei to efficiently polarize target samples in contact
    with the diamond crystal.},
  bdsk-url-1={https://www.pnas.org/content/116/37/18334},
  bdsk-url-2={https://doi.org/10.1073/pnas.1908780116},
  doi={10.1073/pnas.1908780116},
  publisher={National Academy of Sciences},
  url={https://www.pnas.org/content/116/37/18334}
}

@Article{Broadway2018,
  author={Broadway, David A and Tetienne, Jean-Philippe and Stacey, Alastair and
    Wood, James DA and Simpson, David A and Hall, Liam T and Hollenberg, Lloyd
    CL},
  journal={Nat. Commun.},
  title={Quantum probe hyperpolarisation of molecular nuclear spins},
  year={2018},
  pages={1246},
  volume={9},
  bdsk-url-1={https://doi.org/10.1038/s41467-018-03578-1},
  doi={https://doi.org/10.1038/s41467-018-03578-1},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41467-018-03578-1}
}

@Article{Tran2016,
  author={Tran, Toan Trong and Bray, Kerem and Ford, Michael J and Toth, Milos
    and Aharonovich, Igor},
  journal={Nat. Nanotechnol.},
  title={Quantum emission from hexagonal boron nitride monolayers},
  year={2016},
  number={1},
  pages={37--41},
  volume={11},
  bdsk-url-1={https://doi.org/10.1038/nnano.2015.242},
  doi={https://doi.org/10.1038/nnano.2015.242},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nnano.2015.242}
}

@Article{Sajid2020,
  author={A Sajid and Michael J Ford and Jeffrey R Reimers},
  journal={Rep. Progr. Phys.},
  title={Single-photon emitters in hexagonal boron nitride: a review of progress},
  year={2020},
  month={mar},
  number={4},
  pages={044501},
  volume={83},
  bdsk-url-1={https://doi.org/10.1088/1361-6633/ab6310},
  doi={10.1088/1361-6633/ab6310},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/1361-6633/ab6310}
}

@article{Gyamfi2019,
  author={Gyamfi, JA},
  journal={arXiv preprint arXiv:1907.07122},
  title={An Introduction to the Holstein-Primakoff Transformation, with Applications
    in Magnetic Resonance},
  url={https://arxiv.org/abs/1907.07122},
  year={2019},
  bdsk-url-1={https://arxiv.org/abs/1907.07122}
}

@article{Abad2016,
  author={Abad, Tahereh and Karimipour, Vahid},
  doi={10.1103/PhysRevB.93.195127},
  issue={19},
  journal={Phys. Rev. B},
  month={May},
  numpages={5},
  pages={195127},
  publisher={American Physical Society},
  title={Scaling of macroscopic superpositions close to a quantum phase transition},
  url={https://link.aps.org/doi/10.1103/PhysRevB.93.195127},
  volume={93},
  year={2016},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.93.195127},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.93.195127}
}

@Article{Lieb1961,
  author={Elliott Lieb and Theodore Schultz and Daniel Mattis},
  journal={Ann. Phys.},
  title={Two soluble models of an antiferromagnetic chain},
  year={1961},
  issn={0003-4916},
  number={3},
  pages={407-466},
  volume={16},
  abstract={Two genuinely quantum mechanical models for an antiferromagnetic linear
    chain with nearest neighbor interactions are constructed and solved exactly,
    in the sense that the ground state, all the elementary excitations and the
    free energy are found. A general formalism for calculating the instantaneous
    correlation between any two spins is developed and applied to the investigation
    of short- and long-range order. Both models show nonvanishing long-range order
    in the ground state for a range of values of a certain parameter {\^I}{\guillemotright}
    which is analogous to an anisotropy parameter in the Heisenberg model. A detailed
    comparison with the Heisenberg model suggests that the latter has no long-range
    order in the isotropic case but finite long-range order for any finite amount
    of anisotropy. The unreliability of variational methods for determining long-range
    order is emphasized. It is also shown that for spin 12 systems having rather
    general isotropic Heisenberg interactions favoring an antiferromagnetic ordering,
    the ground state is nondegenerate and there is no energy gap above the ground
    state in the energy spectrum of the total system.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/0003491661901154},
  bdsk-url-2={https://doi.org/10.1016/0003-4916(61)90115-4},
  date-modified={2022-05-15 08:41:30 +0430},
  doi={https://doi.org/10.1016/0003-4916(61)90115-4},
  url={https://www.sciencedirect.com/science/article/pii/0003491661901154}
}

@Article{Pfeuty1970,
  author={Pierre Pfeuty},
  journal={Ann. Phys.},
  title={The one-dimensional Ising model with a transverse field},
  year={1970},
  issn={0003-4916},
  number={1},
  pages={79-90},
  volume={57},
  abstract={The one-dimensional Ising model with a transverse field is solved exactly
    by transforming the set of Pauli operators to a new set of Fermi operators.
    The elementary excitations, the ground-state energy and the free energy are
    found. The instantaneous correlation function between any two spins is calculated
    and this model shows a finite long-range order in the ground state when the
    transverse field is less than a critical value.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/0003491670902708},
  bdsk-url-2={https://doi.org/10.1016/0003-4916(70)90270-8},
  date-modified={2022-05-15 08:41:52 +0430},
  doi={https://doi.org/10.1016/0003-4916(70)90270-8},
  url={https://www.sciencedirect.com/science/article/pii/0003491670902708}
}

@Article{Cassabois2016,
  author={Cassabois, Guillaume and Valvin, Pierre and Gil, Bernard},
  journal={Nat. Photonics},
  title={Hexagonal boron nitride is an indirect bandgap semiconductor},
  year={2016},
  number={4},
  pages={262--266},
  volume={10},
  bdsk-url-1={https://doi.org/10.1038/nphoton.2015.277},
  date-modified={2022-05-15 08:39:20 +0430},
  doi={https://doi.org/10.1038/nphoton.2015.277},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nphoton.2015.277}
}

@article{healey2021q,
  author={Healey, AJ and Scholten, SC and Yang, T and Scott, JA and Abrahams, GJ
    and Robertson, IO and Hou, XF and Guo, YF and Rahman, S and Lu, Y and others},
  journal={arXiv preprint arXiv:2112.03488},
  title={Quantum microscopy with van der Waals heterostructures},
  url={https://arxiv.org/abs/2112.03488},
  year={2021}
}

@Article{Tetienne2021b,
  author={Tetienne, J.-P.},
  journal={Nat. Phys.},
  title={Quantum sensors go flat},
  year={2021},
  number={10},
  pages={1074--1075},
  volume={17},
  bdsk-url-1={https://doi.org/10.1038/s41567-021-01338-5},
  date-modified={2022-05-15 08:42:57 +0430},
  doi={https://doi.org/10.1038/s41567-021-01338-5},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41567-021-01338-5}
}

@article{Geim2013,
  author={Geim, Andre K and Grigorieva, Irina V},
  date-modified={2022-05-15 08:40:36 +0430},
  doi={https://doi.org/10.1038/nature12385},
  journal={Nature},
  number={7459},
  pages={419--425},
  publisher={Nature Publishing Group},
  title={Van der Waals heterostructures},
  url={https://doi.org/10.1038/nature12385},
  volume={499},
  year={2013},
  bdsk-url-1={https://doi.org/10.1038/nature12385}
}

@Article{Novoselov2016,
  author={K. S. Novoselov and A. Mishchenko and A. Carvalho and A. H. Castro Neto},
  journal={Science},
  title={2D materials and van der Waals heterostructures},
  year={2016},
  number={6298},
  pages={9439},
  volume={353},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/science.aac9439},
  bdsk-url-2={https://doi.org/10.1126/science.aac9439},
  date-modified={2022-05-15 09:05:08 +0430},
  doi={10.1126/science.aac9439},
  url={https://www.science.org/doi/abs/10.1126/science.aac9439}
}

@article{Gong2017,
  author={Gong, Cheng and Li, Lin and Li, Zhenglu and Ji, Huiwen and Stern, Alex
    and Xia, Yang and Cao, Ting and Bao, Wei and Wang, Chenzhe and Wang, Yuan and
    others},
  date-modified={2022-05-15 08:40:41 +0430},
  doi={https://doi.org/10.1038/nature22060},
  journal={Nature},
  number={7657},
  pages={265--269},
  publisher={Nature Publishing Group},
  title={Discovery of intrinsic ferromagnetism in two-dimensional van der Waals
    crystals},
  url={https://doi.org/10.1038/nature22060},
  volume={546},
  year={2017},
  bdsk-url-1={https://doi.org/10.1038/nature22060}
}

@article{huang2017,
  author={Huang, Bevin and Clark, Genevieve and Navarro-Moratalla, Efr{\'e}n and
    Klein, Dahlia R and Cheng, Ran and Seyler, Kyle L and Zhong, Ding and Schmidgall,
    Emma and McGuire, Michael A and Cobden, David H and others},
  doi={https://doi.org/10.1038/nature22391},
  journal={Nature},
  number={7657},
  pages={270--273},
  publisher={Nature Publishing Group},
  title={Layer-dependent ferromagnetism in a van der Waals crystal down to the
    monolayer limit},
  url={https://doi.org/10.1038/nature22391},
  volume={546},
  year={2017},
  bdsk-url-1={https://doi.org/10.1038/nature22391}
}

@Article{Li2019,
  author={Li, Hui and Ruan, Shuangchen and Zeng, Yu-Jia},
  journal={Adv. Mater.},
  title={Intrinsic Van Der Waals Magnetic Materials from Bulk to the 2D Limit:
    New Frontiers of Spintronics},
  year={2019},
  number={27},
  pages={1900065},
  volume={31},
  abstract={Abstract 2D van der Waals (vdW) magnets, which present intrinsic ferromagnetic/antiferromagnetic
    ground states at finite temperatures down to atomic-layer thicknesses, open
    a new horizon in materials science and enable the potential development of
    new spin-related applications. The layered structure of vdW magnets facilitates
    their atomic-layer cleavability and magnetic anisotropy, which counteracts
    spin fluctuations, thereby providing an ideal platform for theoretically and
    experimentally exploring magnetic phase transitions in the 2D limit. With reduced
    dimensions, the susceptibility of 2D magnets to a large variety of external
    stimuli also makes them more promising than their bulk counterpart in various
    device applications. Here, the current status of characterization and tuning
    of the magnetic properties of 2D vdW magnets, particularly the atomic-layer
    thickness, is presented. Various state-of-the-art optical and electrical techniques
    have been applied to reveal the magnetic states of 2D vdW magnets. Other emerging
    2D vdW magnets and future perspectives on the stacking strategy are also given;
    it is believed that they will excite more intensive research and provide unprecedented
    opportunities in the field of spintronics.},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201900065},
  bdsk-url-2={https://doi.org/10.1002/adma.201900065},
  date-modified={2022-05-15 08:41:22 +0430},
  doi={https://doi.org/10.1002/adma.201900065},
  keywords={2D vdW magnets, exfoliation, ferromagnetism, spintronics},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201900065}
}

@Article{Liu2020,
  author={Liu, Shanshan and Yang, Ke and Liu, Wenqing and Zhang, Enze and Li, Zihan
    and Zhang, Xiaoqian and Liao, Zhiming and Zhang, Wen and Sun, Jiabao and Yang,
    Yunkun and others},
  journal={Natl. Sci. Rev.},
  title={Two-dimensional ferromagnetic superlattices},
  year={2020},
  number={4},
  pages={745--754},
  volume={7},
  bdsk-url-1={https://doi.org/10.1093/nsr/nwz205},
  date-modified={2022-05-15 08:41:39 +0430},
  doi={https://doi.org/10.1093/nsr/nwz205},
  publisher={Oxford University Press},
  url={https://doi.org/10.1093/nsr/nwz205}
}

@article{koehl2011,
  title={Room temperature coherent control of defect spin qubits in silicon carbide},
  author={Koehl, William F and Buckley, Bob B and Heremans, F Joseph and Calusine,
    Greg and Awschalom, David D},
  journal={Nature},
  volume={479},
  number={7371},
  pages={84--87},
  year={2011},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature10562}
}

@article{widmann2015,
  title={Coherent control of single spins in silicon carbide at room temperature},
  author={Widmann, Matthias and Lee, Sang-Yun and Rendler, Torsten and Son, Nguyen
    Tien and Fedder, Helmut and Paik, Seoyoung and Yang, Li-Ping and Zhao, Nan
    and Yang, Sen and Booker, Ian and others},
  journal={Nat. Mater.},
  volume={14},
  number={2},
  pages={164--168},
  year={2015},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nmat4145}
}

@article{Falk2015,
  title={Optical Polarization of Nuclear Spins in Silicon Carbide},
  author={Falk, Abram L. and Klimov, Paul V. and Iv\'ady, Viktor and Sz\'asz, Kriszti\'an
    and Christle, David J. and Koehl, William F. and Gali, \'Ad\'am and Awschalom,
    David D.},
  journal={Phys. Rev. Lett.},
  volume={114},
  issue={24},
  pages={247603},
  numpages={6},
  year={2015},
  month={Jun},
  publisher={American Physical Society},
  doi={10.1103/PhysRevLett.114.247603},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.114.247603}
}

@book{Baxter,
  title={Exactly solved models in statistical mechanics},
  author={R.J. Baxter},
  year={1982},
  publisher={London, Academic Press}
}

@book{nolting,
  title={Quantum theory of magnetism},
  author={Nolting, Wolfgang and Ramakanth, Anupuru},
  year={2009},
  publisher={Springer Science {\&} Business Media}
}

@Article{dolde2014high,
  author={Dolde, Florian and Bergholm, Ville and Wang, Ya and Jakobi, Ingmar and
    Naydenov, Boris and Pezzagna, S{\'e}bastien and Meijer, Jan and Jelezko, Fedor
    and Neumann, Philipp and Schulte-Herbr{\"u}ggen, Thomas and others},
  journal={Nat. Commun.},
  title={High-fidelity spin entanglement using optimal control},
  year={2014},
  number={1},
  pages={3371},
  volume={5},
  doi={https://doi.org/10.1038/ncomms4371},
  publisher={Nature Publishing Group}
}

@article{haykal2022,
  title={Decoherence of $\rm{V_B}$ spin defects in monoisotopic hexagonal boron
    nitride},
  author={Haykal, Angela and Tanos, Rana and Minotto, Noel and Durand, Alrik and
    Fabre, Florentin and Li, Jiahan and Edgar, JH and Ivady, Viktor and Gali, Adam
    and Michel, Thierry and others},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={1--7},
  year={2022},
  doi={https://doi.org/10.1038/s41467-022-31743-0},
  publisher={Nature Publishing Group}
}

@article{Gottscholl2021,
  author={Andreas Gottscholl and Matthias Diez and Victor Soltamov and Christian
    Kasper and Andreas Sperlich and Mehran Kianinia and Carlo Bradac and Igor Aharonovich
    and Vladimir Dyakonov },
  title={Room temperature coherent control of spin defects in hexagonal boron nitride},
  journal={Science Advances},
  volume={7},
  number={14},
  pages={eabf3630},
  year={2021},
  doi={10.1126/sciadv.abf3630},
  URL={https://www.science.org/doi/abs/10.1126/sciadv.abf3630}
}

@article{Liu2022,
  title={Coherent dynamics of multi-spin $\rm{V_B^-}$ centers in hexagonal boron
    nitride},
  author={Liu, Wei and Iv{\'a}dy, Viktor and Li, Zhi-Peng and Yang, Yuan-Ze and
    Yu, Shang and Meng, Yu and Wang, Zhao-An and Guo, Nai-Jie and Yan, Fei-Fei
    and Li, Qiang and others},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={1--8},
  year={2022},
  url={https://doi.org/10.1038/s41467-022-33399-2},
  publisher={Nature Publishing Group}
}

@article{Gao2021,
  author={Gao, Xingyu and Jiang, Boyang and Llacsahuanga Allcca, Andres E. and
    Shen, Kunhong and Sadi, Mohammad A. and Solanki, Abhishek B. and Ju, Peng and
    Xu, Zhujing and Upadhyaya, Pramey and Chen, Yong P. and Bhave, Sunil A. and
    Li, Tongcang},
  title={High-Contrast Plasmonic-Enhanced Shallow Spin Defects in Hexagonal Boron
    Nitride for Quantum Sensing},
  doi={10.1021/acs.nanolett.1c02495},
  journal={Nan. Lett.},
  volume={21},
  number={18},
  pages={7708-7714},
  year={2021},
  URL={https://doi.org/10.1021/acs.nanolett.1c02495 }
}

@article{ye2019spin,
  title={Spin coherence in two-dimensional materials},
  author={Ye, Meng and Seo, Hosung and Galli, Giulia},
  doi={https://doi.org/10.1038/s41524-019-0182-3},
  journal={npj Computational Materials},
  volume={5},
  number={1},
  pages={1--6},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{Liu_2022,
  doi={10.1088/2633-4356/ac7e9f},
  url={https://doi.org/10.1088/2633-4356/ac7e9f},
  year={2022},
  month={jul},
  publisher={{IOP} Publishing},
  volume={2},
  number={3},
  pages={032002},
  author={Wei Liu and Nai-Jie Guo and Shang Yu and Yu Meng and Zhi-Peng Li and
    Yuan-Ze Yang and Zhao-An Wang and Xiao-Dong Zeng and Lin-Ke Xie and Qiang Li
    and Jun-Feng Wang and Jin-Shi Xu and Yi-Tao Wang and Jian-Shun Tang and Chuan-Feng
    Li and Guang-Can Guo},
  title={Spin-active defects in hexagonal boron nitride},
  journal={Materials for Quantum Technology}
}

@article{lee2022first,
  title={First-principles theory of extending the spin qubit coherence time in
    hexagonal boron nitride},
  author={Lee, Jaewook and Park, Huijin and Seo, Hosung},
  doi={https://doi.org/10.1038/s41699-022-00336-2},
  journal={npj 2D Mater Appl},
  volume={6},
  number={60},
  pages={60},
  year={2022}
}

@article{gottscholl_2020n,
  title={Initialization and read-out of intrinsic spin defects in a van der Waals
    crystal at room temperature},
  author={Gottscholl, Andreas and Kianinia, Mehran and Soltamov, Victor and Orlinskii,
    Sergei and Mamin, Georgy and Bradac, Carlo and Kasper, Christian and Krambrock,
    Klaus and Sperlich, Andreas and Toth, Milos and others},
  doi={https://doi.org/10.1038/s41563-020-0619-6},
  journal={Nat. Mater.},
  volume={19},
  number={5},
  pages={540--545},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{baber2022,
  author={Baber, Simon and Malein, Ralph Nicholas Edward and Khatri, Prince and
    Keatley, Paul Steven and Guo, Shi and Withers, Freddie and Ramsay, Andrew J.
    and Luxmoore, Isaac J.},
  title={Excited State Spectroscopy of Boron Vacancy Defects in Hexagonal Boron
    Nitride Using Time-Resolved Optically Detected Magnetic Resonance},
  journal={Nano. Lett.},
  volume={22},
  number={1},
  pages={461-467},
  year={2022},
  doi={10.1021/acs.nanolett.1c04366},
  URL={https://doi.org/10.1021/acs.nanolett.1c04366 }
}

@article{Yu2022,
  author={Yu, Pei and Sun, Haoyu and Wang, Mengqi and Zhang, Tao and Ye, Xiangyu
    and Zhou, Jingwei and Liu, Hangyu and Wang, Cheng-Jie and Shi, Fazhan and Wang,
    Ya and Du, Jiangfeng},
  title={Excited-State Spectroscopy of Spin Defects in Hexagonal Boron Nitride},
  journal={Nano Letters},
  volume={22},
  number={9},
  pages={3545-3549},
  year={2022},
  doi={10.1021/acs.nanolett.1c04841},
  URL={https://doi.org/10.1021/acs.nanolett.1c04841 }
}

@article{Murzakhanov,
  author={Murzakhanov, Fadis F. and Mamin, Georgy Vladimirovich and Orlinskii,
    Sergei Borisovich and Gerstmann, Uwe and Schmidt, Wolf Gero and Biktagirov,
    Timur and Aharonovich, Igor and Gottscholl, Andreas and Sperlich, Andreas and
    Dyakonov, Vladimir and Soltamov, Victor A.},
  title={Electron-Nuclear Coherent Coupling and Nuclear Spin Readout through Optically
    Polarized $\rm{V_B^-} $Spin States in hBN},
  journal={Nano Letters},
  volume={22},
  number={7},
  pages={2718-2724},
  year={2022},
  doi={10.1021/acs.nanolett.1c04610},
  URL={https://doi.org/10.1021/acs.nanolett.1c04610 }
}

@article{Mu2022,
  title={Excited-State Optically Detected Magnetic Resonance of Spin Defects in
    Hexagonal Boron Nitride},
  author={Mu, Zhao and Cai, Hongbing and Chen, Disheng and Kenny, Jonathan and
    Jiang, Zhengzhi and Ru, Shihao and Lyu, Xiaodan and Koh, Teck Seng and Liu,
    Xiaogang and Aharonovich, Igor and Gao, Weibo},
  journal={Phys. Rev. Lett.},
  volume={128},
  issue={21},
  pages={216402},
  numpages={6},
  year={2022},
  month={May},
  publisher={American Physical Society},
  doi={10.1103/PhysRevLett.128.216402},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.128.216402}
}

@article{ramsay2022room,
  author={Ramsay, Andrew J and Hekmati, Reza and Patrickson, Charlie J and Baber,
    Simon and Arvidsson-Shukur, David RM and Bennett, Anthony J and Luxmoore, Isaac
    J},
  journal={arXiv preprint arXiv:2205.12747},
  title={Room temperature coherent control of protected qubit in hexagonal boron
    nitride},
  url={https://arxiv.org/abs/2205.12747},
  year={2022}
}

@article{Riedel,
  title={Resonant Addressing and Manipulation of Silicon Vacancy Qubits in Silicon
    Carbide},
  author={Riedel, D. and Fuchs, F. and Kraus, H. and V{\"a}th, S. and Sperlich,
    A. and Dyakonov, V. and Soltamova, A. A. and Baranov, P. G. and Ilyin, V. A.
    and Astakhov, G. V.},
  journal={Phys. Rev. Lett.},
  volume={109},
  issue={22},
  pages={226402},
  numpages={5},
  year={2012},
  month={Nov},
  publisher={American Physical Society},
  doi={10.1103/PhysRevLett.109.226402},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.109.226402}
}

@article{koehl2011room,
  title={Room temperature coherent control of defect spin qubits in silicon carbide},
  author={Koehl, William F and Buckley, Bob B and Heremans, F Joseph and Calusine,
    Greg and Awschalom, David D},
  journal={Nature},
  volume={479},
  number={7371},
  pages={84--87},
  year={2011},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature10562}
}

@article{DOHERTY20131,
  title={The nitrogen-vacancy colour centre in diamond},
  journal={Physics Reports},
  volume={528},
  number={1},
  pages={1-45},
  year={2013},
  issn={0370-1573},
  doi={https://doi.org/10.1016/j.physrep.2013.02.001},
  url={https://www.sciencedirect.com/science/article/pii/S0370157313000562},
  author={Marcus W. Doherty and Neil B. Manson and Paul Delaney and Fedor Jelezko
    and J{\"o}rg Wrachtrup and Lloyd C.L. Hollenberg}
}

@article{Castelletto_2020,
  doi={10.1088/2515-7647/ab77a2},
  url={https://doi.org/10.1088/2515-7647/ab77a2},
  year={2020},
  month={mar},
  publisher={{IOP} Publishing},
  volume={2},
  number={2},
  pages={022001},
  author={Stefania Castelletto and Alberto Boretti},
  title={Silicon carbide color centers for quantum applications},
  journal={Journal of Physics: Photonics}
}

@article{liu20192d,
  title={2D materials for quantum information science},
  author={Liu, Xiaolong and Hersam, Mark C},
  journal={Nature Reviews Materials},
  volume={4},
  number={10},
  pages={669--684},
  year={2019},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/s41578-019-0136-x}
}

@article{liu2016van,
  title={Van der Waals heterostructures and devices},
  author={Liu, Yuan and Weiss, Nathan O and Duan, Xidong and Cheng, Hung-Chieh
    and Huang, Yu and Duan, Xiangfeng},
  journal={Nature Reviews Materials},
  volume={1},
  number={9},
  pages={1--17},
  year={2016},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/natrevmats.2016.42}
}

@article{waldherr2014,
  title={Quantum error correction in a solid-state hybrid spin register},
  author={Waldherr, Gerald and Wang, Ya and Zaiser, S and Jamali, M and Schulte-Herbr{\"u}ggen,
    T and Abe, H and Ohshima, T and Isoya, J and Du, JF and Neumann, P and others},
  journal={Nature},
  volume={506},
  number={7487},
  pages={204--207},
  year={2014},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature12919}
}

@article{Pompili,
  author={M. Pompili and S. L. N. Hermans and S. Baier and H. K. C. Beukers and
    P. C. Humphreys and R. N. Schouten and R. F. L. Vermeulen and M. J. Tiggelman
    and L. dos Santos Martins and B. Dirkse and S. Wehner and R. Hanson },
  title={Realization of a multinode quantum network of remote solid-state qubits},
  journal={Science},
  volume={372},
  number={6539},
  pages={259-264},
  year={2021},
  doi={10.1126/science.abg1919},
  URL={https://www.science.org/doi/abs/10.1126/science.abg1919}
}

@article{Weber,
  author={J. R. Weber and W. F. Koehl and J. B. Varley and A. Janotti and B. B.
    Buckley and C. G. Van de Walle and D. D. Awschalom },
  title={Quantum computing with defects},
  journal={Proceedings of the National Academy of Sciences},
  volume={107},
  number={19},
  pages={8513-8518},
  year={2010},
  doi={10.1073/pnas.1003052107},
  URL={https://www.pnas.org/doi/abs/10.1073/pnas.1003052107}
}

@article{Bradley2019,
  title={A Ten-Qubit Solid-State Spin Register with Quantum Memory up to One Minute},
  author={Bradley, C. E. and Randall, J. and Abobeih, M. H. and Berrevoets, R.
    C. and Degen, M. J. and Bakker, M. A. and Markham, M. and Twitchen, D. J. and
    Taminiau, T. H.},
  journal={Phys. Rev. X},
  volume={9},
  issue={3},
  pages={031045},
  numpages={12},
  year={2019},
  month={Sep},
  publisher={American Physical Society},
  doi={10.1103/PhysRevX.9.031045},
  url={https://link.aps.org/doi/10.1103/PhysRevX.9.031045}
}

@article{Schirhagl,
  author={Schirhagl, Romana and Chang, Kevin and Loretz, Michael and Degen, Christian
    L.},
  title={Nitrogen-Vacancy Centers in Diamond: Nanoscale Sensors for Physics and
    Biology},
  journal={Annual Review of Physical Chemistry},
  volume={65},
  number={1},
  pages={83-105},
  year={2014},
  doi={10.1146/annurev-physchem-040513-103659},
  URL={https://doi.org/10.1146/annurev-physchem-040513-103659 }
}

@article{awschalom2018,
  title={Quantum technologies with optically interfaced solid-state spins},
  author={Awschalom, David D and Hanson, Ronald and Wrachtrup, J{\"o}rg and Zhou,
    Brian B},
  journal={Nature Photonics},
  volume={12},
  number={9},
  pages={516--527},
  year={2018},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/s41566-018-0232-2}
}

@article{atature2018,
  title={Material platforms for spin-based photonic quantum technologies},
  author={Atat{\"u}re, Mete and Englund, Dirk and Vamivakas, Nick and Lee, Sang-Yun
    and Wrachtrup, Joerg},
  journal={Nature Reviews Materials},
  volume={3},
  number={5},
  pages={38--51},
  year={2018},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/s41578-018-0008-9}
}

@article{Graham,
  author={Graham, Michael J. and Zadrozny, Joseph M. and Fataftah, Majed S. and
    Freedman, Danna E.},
  title={Forging Solid-State Qubit Design Principles in a Molecular Furnace},
  journal={Chemistry of Materials},
  volume={29},
  number={5},
  pages={1885-1897},
  year={2017},
  doi={10.1021/acs.chemmater.6b05433},
  URL={https://doi.org/10.1021/acs.chemmater.6b05433 }
}

@article{Degen2017,
  title={Quantum sensing},
  author={Degen, C. L. and Reinhard, F. and Cappellaro, P.},
  journal={Rev. Mod. Phys.},
  volume={89},
  issue={3},
  pages={035002},
  numpages={39},
  year={2017},
  month={Jul},
  publisher={American Physical Society},
  doi={10.1103/RevModPhys.89.035002},
  url={https://link.aps.org/doi/10.1103/RevModPhys.89.035002}
}

@article{divincenzo2000,
  title={The physical implementation of quantum computation},
  author={DiVincenzo, David P},
  journal={Fortschritte der Physik: Progress of Physics},
  volume={48},
  number={9-11},
  pages={771--783},
  year={2000},
  publisher={Wiley Online Library},
  url={https://doi.org/10.1002/1521-3978(200009)48:9/11<771::AID-PROP771>3.0.CO;2-E},
  doi={https://doi.org/10.1002/1521-3978(200009)48:9/11<771::AID-PROP771>3.0.CO;2-E}
}

@article{Hahn,
  title={Spin Echoes},
  author={Hahn, E. L.},
  journal={Phys. Rev.},
  volume={80},
  issue={4},
  pages={580--594},
  numpages={0},
  year={1950},
  month={Nov},
  publisher={American Physical Society},
  doi={10.1103/PhysRev.80.580},
  url={https://link.aps.org/doi/10.1103/PhysRev.80.580}
}

@article{Novoselov,
  author={K. S. Novoselov and A. Mishchenko and A. Carvalho and A. H. Castro Neto
    },
  title={2D materials and van der Waals heterostructures},
  journal={Science},
  volume={353},
  number={6298},
  pages={aac9439},
  year={2016},
  doi={10.1126/science.aac9439},
  URL={https://www.science.org/doi/abs/10.1126/science.aac9439}
}

@article{balasubramanian2009,
  title={Ultralong spin coherence time in isotopically engineered diamond},
  author={Balasubramanian, Gopalakrishnan and Neumann, Philipp and Twitchen, Daniel
    and Markham, Matthew and Kolesov, Roman and Mizuochi, Norikazu and Isoya, Junichi
    and Achard, Jocelyn and Beck, Johannes and Tissler, Julia and others},
  journal={Nature materials},
  volume={8},
  number={5},
  pages={383--387},
  year={2009},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nmat2420}
}

@article{widmann2015,
  title={Coherent control of single spins in silicon carbide at room temperature},
  author={Widmann, Matthias and Lee, Sang-Yun and Rendler, Torsten and Son, Nguyen
    Tien and Fedder, Helmut and Paik, Seoyoung and Yang, Li-Ping and Zhao, Nan
    and Yang, Sen and Booker, Ian and others},
  journal={Nature materials},
  volume={14},
  number={2},
  pages={164--168},
  year={2015},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nmat4145}
}

@article{Zhang2017,
  title={Depth-dependent decoherence caused by surface and external spins for NV
    centers in diamond},
  author={Zhang, Wenlong and Zhang, Jian and Wang, Junfeng and Feng, Fupan and
    Lin, Shengran and Lou, Liren and Zhu, Wei and Wang, Guanzhong},
  journal={Phys. Rev. B},
  volume={96},
  issue={23},
  pages={235443},
  numpages={7},
  year={2017},
  month={Dec},
  publisher={American Physical Society},
  doi={10.1103/PhysRevB.96.235443},
  url={https://link.aps.org/doi/10.1103/PhysRevB.96.235443}
}
@article{Maze,
  title = {Spin-lattice relaxation of individual solid-state spins},
  author = {Norambuena, A. and Munoz, E. and Dinani, H. T. and Jarmola, A. and Maletinsky, P. and Budker, D. and Maze, J. R.},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {9},
  pages = {094304},
  numpages = {13},
  year = {2018},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.094304},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.094304}
}

@article{rost,
author = {Rost, Hakon I. and Cooil, Simon P. and Asland, Anna Cecilie and Hu, Jinbang and Ali, Ayaz and Taniguchi, Takashi and Watanabe, Kenji and Belle, Branson D. and Holst, Bodil and Sadowski, Jerzy T. and Mazzola, Federico and Wells, Justin W.},
title = {Phonon-Mediated Quasiparticle Lifetime Renormalizations in Few-Layer Hexagonal Boron Nitride},
journal = {Nano Letters},
volume = {23},
number = {16},
pages = {7539-7545},
year = {2023},
doi = {10.1021/acs.nanolett.3c02086},
URL = { https://doi.org/10.1021/acs.nanolett.3c02086}
}

@article{Tabesh2023,
  title = {Active hyperpolarization of the nuclear spin lattice: Application to hexagonal boron nitride color centers},
  author = {Tabesh, F. T. and Fani, M. and Pedernales, J. S. and Plenio, M. B. and Abdi, M.},
  journal = {Phys. Rev. B},
  volume = {107},
  issue = {21},
  pages = {214307},
  numpages = {12},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.107.214307},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.107.214307}
}


@article{Tabesh_2022,
doi = {10.1088/2058-9565/ac2f4d},
url = {https://dx.doi.org/10.1088/2058-9565/ac2f4d},
year = {2021},
month = {oct},
publisher = {IOP Publishing},
volume = {7},
number = {1},
pages = {015002},
author = {F T Tabesh and Q Hassanzada and M Hadian and A Hashemi and I Abdolhosseini Sarsari and M Abdi},
title = {Strain induced coupling and quantum information processing with hexagonal boron nitride quantum emitters},
journal = {Quantum Science and Technology},
}

@misc{jafari2024,
      title={Characterizing Noise of Driven Controlled Field Using the Central Spin Model}, 
      author={R. Jafari and A. Asadian and M. Abdi and Alireza Akbari},
      year={2024},
      eprint={2409.01375},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2409.01375},    
}

@article{SHAYEGANI2024129966,
	title = {Dephasing dynamics of a central spin interacting with a classical Ising spin bath},
	journal = {Physics Letters A},
	volume = {526},
	pages = {129966},
	year = {2024},
	issn = {0375-9601},
	doi = {https://doi.org/10.1016/j.physleta.2024.129966},
	url = {https://www.sciencedirect.com/science/article/pii/S0375960124006601},
	author = {Fariba Shayegani and Keivan {Aghababaei Samani} and Mehdi Abdi and Mohammad Walid AlMasri},
}

@Comment{jabref-meta: databaseType:bibtex;}


